Wavelet-Based Multiscale Flow For Realistic Image Deformation in the Large Diffeomorphic Deformation Model Framework

Estimating accurate high-dimensional transformations remains very challenging, especially in a clinical setting. In this paper, we introduce a multiscale parameterization of deformations to enhance registration and atlas estimation in the Large Deformation Diffeomorphic Metric Mapping framework. Using the Haar wavelet transform, a multiscale representation of the initial velocity fields is computed to optimize transformations in a coarse-to-fine fashion. This additional layer of spatial regularization does not modify the underlying model of deformations. As such, it preserves the original kernel Hilbert space structure of the velocity fields, enabling the algorithm to perform efficient gradient descent. Numerical experiments on several datasets, including abnormal fetal brain images, show that compared to the original algorithm, the coarse-to-fine strategy reaches higher performance and yields template images that preserve important details while avoiding unrealistic features. This highly versatile strategy can easily be applied to other mathematical frameworks for almost no additional computational cost.

==> Risser_.tex <==
\begin{table}[t]
    \caption{\rev {Performance of the original LDDMM and the LDDMM combined with multiscale optimization in the toy experiment. Each algorithm is evaluated with different kernel sizes $\sigma_g$. The multiscale algorithm is tested with different initial scales $S_0$, ranging from $S_{max}$ to 2. The presented values are the total residuals values between $I_s$ and $I_t$ in the image domain and a ROI covering the indentation, standard deviation of the Jacobian determinant and algorithm runtime (RT) (in minute).}}
    \centering
\small
\begin{simpletabular}{@{}cc|cccc@{}}
\multicolumn{6}{c}{\textbf{LDDMM (Deformetrica version)}}\\
\toprule
 $\sigma_g$ & $k_g$ & $\Delta_{J}$ & $\Delta_{J}(\text{\footnotesize ROI})$ & SD(J) & RT\\
\midrule
20 & 9 & 17.05 & 8.0 & 0.05 & 0.27 \\
15 & 16 & 16.81 & 8.0 & 0.05 & 0.38 \\
10 & 25 & 15.05 & 8.0 & 0.07 & 0.43\\
7 & 64 & 11.52 & 6.67 & 0.09 & 0.4 \\
3 & 289 & 1.30 & 0.31 & 0.19 &0.28\\
2.5 & 400 & 1.49 & 0.11 & 0.24 & 0.35 \\
2 & 625 & 0.37 & 0.09 & 0.27 & 0.58 \\ % 2.8 = 0.50
1.7 & 841 & 9.36 & 0.03 & 0.23 & 0.33 \\ % 2.8 = 0.50

\midrule
\multicolumn{6}{c}{\textbf{LDDMM (Risser et al. version)}}\\
\midrule
1 & & 0.39 & 0.07 & 0.07 & \\
\bottomrule
\end{simpletabular}

\vspace{0.5cm}
\begin{simpletabular}{@{}ccc|cccc@{}}
\multicolumn{7}{c}{\textbf{LDDMM $+$ Multiscale}}\\
\toprule
 $\sigma_g$ & $k_g$ & $S_0$ & $\Delta_{J}$ & $\Delta_{J}({\text{\footnotesize ROI}})$ & SD(J) & RT \\
   \midrule
\multirow{3}{*}{7}  & \multirow{3}{*}{64} 
&3 & \textbf{11.06} & \textbf{6.45} & 0.11 & 0.72\\
& & 2 & 11.28 & 6.68 & \textbf{0.09} & 0.51 \\
& & 1 & 11.52 & 6.67 & \textbf{0.09}& \textbf{0.4} \\

  \midrule
\multirow{5}{*}{3}  & \multirow{5}{*}{289} 
& 5 & 1.29 & 0.06 & \textbf{0.16} & 1.03 \\
&& 4 & \textbf{0.52} & \textbf{0.03} & \textbf{0.16} & 0.98 \\
&  &3 & 0.59 & 0.07 & 0.22 & 0.93\\
& & 2 & 0.90 & 0.11 & 0.23 & 0.65 \\ % 0.23
&  & 1 & 1.30 & 0.31 & 0.19 &\textbf{0.28}\\

 \midrule
\multirow{5}{*}{2.5}  & \multirow{5}{*}{400} 
& 5 & 0.44 & \textbf{0.04}  & 0.29 & 1.23 \\
&& 4 & \textbf{0.37} & 0.05 & \textbf{0.23} & 1.12 \\
&  &3 & 0.47 & 0.06&0.26 & 0.93\\
& & 2 & 0.65 & 0.06 & 0.29& 0.51 \\
& & 1 & 1.49 & 0.11 & 0.24 & \textbf{0.35} \\

\midrule
\multirow{5}{*}{2}  & \multirow{5}{*}{625} 
& 5 & 0.43 & 0.06 & 0.29 & 1.66 \\
&& 4 & \textbf{0.20} & \textbf{0.02}& \textbf{0.21} & 1.45 \\
&  &3 & 0.47 & 0.06& 0.26 & 1.10\\
& & 2 & 0.59 & 0.12 & 0.24 & 0.63 \\
&& 1 & 0.37 & 0.09 & 0.27 & \textbf{0.58} \\ % 2.8 = 0.50

\midrule
\multirow{5}{*}{1.7}  & \multirow{5}{*}{841} 
& 5 &4.17 & 0.11 & 0.25 & 1.71 \\
&& 4 & \textbf{1.21} &\textbf{0.0}& 0.24& 1.13 \\
&  &3 &1.26&\textbf{0.0} & 0.24 & 0.97\\
& & 2 & 3.58&0.05& 0.23 & 0.50 \\
&& 1 & 9.36 & 0.03 & \textbf{0.23} & \textbf{0.33} \\ % 2.8 = 0.50

\midrule
\multicolumn{6}{c}{\textbf{Multikernel LDDMM}}\\
\multicolumn{6}{c}{\textbf{MK}}\\
\bottomrule
\end{simpletabular}

\label{table:risser}
\end{table}

